Warping of Radar Data into Camera Image for Cross-Modal Supervision in Automotive Applications

We present an approach to automatically generate semantic labels for real recordings of automotive range-Doppler (RD) radar spectra. Such labels are required when training a neural network for object recognition from radar data. The automatic labeling approach rests on the simultaneous recording of camera and lidar data in addition to the radar spectrum. By warping radar spectra into the camera image, state-of-the-art object recognition algorithms can be applied to label relevant objects, such as cars, in the camera image. The warping operation is designed to be fully differentiable, which allows backpropagating the gradient computed on the camera image through the warping operation to the neural network operating on the radar data. As the warping operation relies on accurate scene flow estimation, we further propose a novel scene flow estimation algorithm which exploits information from camera, lidar and radar sensors. The proposed scene flow estimation approach is compared against a state-of-the-art scene flow algorithm, and it outperforms it by approximately 30% w.r.t. mean average error. The feasibility of the overall framework for automatic label generation for RD spectra is verified by evaluating the performance of neural networks trained with the proposed framework for Direction-of-Arrival estimation.

==> Flowchart_nn_and_gt3.tex <==
% Flowchart of Lidar2RAdar generation
\tikzstyle{decision} = [diamond, draw, fill=gray!20, 
    text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=gray!20, 
    text width=15em, text centered, minimum height=4em]
    \tikzstyle{blockstart} = [rectangle, draw, fill=blue!20, 
    text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{line2} = [draw]
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
    \tikzstyle{block2} = [rectangle, draw, fill=gray!20, 
    text width=13em, text centered, minimum height=4em]
  %\centering 
  
  
  
\tikzstyle{DataInput} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=1cm, text centered, draw=black, fill=gray!30]  

\tikzstyle{process} = [rectangle, minimum width=1.0cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
   
\tikzstyle{arrow} = [draw, -latex',thick]
\tikzstyle{arrowDashed} = [draw, -latex',thick, dashed]


\tikzstyle{diff} = [circle, minimum width=1.0cm, minimum height=1cm, text centered, draw=black, fill=gray!30]


\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)


\begin{tikzpicture}[node distance = 2cm, auto, scale=0.5]

	\node [DataInput, align=center] (fftData) {radar}; 
	\node [process, left=0.5cm of fftData, , align=center, opacity=.0] (NN) {Neural\\ Network};
	
    
    \pgfmathsetmacro{\cubexo}{0.2}
    \pgfmathsetmacro{\cubeyo}{1.5}
	\pgfmathsetmacro{\cubezo}{1.5}
	
	\pgfmathsetmacro{\cubext}{0.2}
    \pgfmathsetmacro{\cubeyt}{1.25}
	\pgfmathsetmacro{\cubezt}{1.25}
	
	\pgfmathsetmacro{\cubextr}{0.2}
    \pgfmathsetmacro{\cubeytr}{1.0}
	\pgfmathsetmacro{\cubeztr}{1.0}
	
	\newcommand\XEo{-5.5,0.5,0}
	
	%\newcommand\XEo{5,-4,0}
	\newcommand\XEt{-5,0.375,0}
	\newcommand\XEtr{-4.5, 0.25, 0}
	
	\newcommand\XDo{-4, 0.25, 0}
	\newcommand\XDt{-3.5,0.375,0}
	\newcommand\XDtr{-3,0.5,0}

\draw[gray,fill=yellow] (\XEo) -- ++(-\cubexo,0, 0) -- ++(0,-\cubeyo,0) -- ++(\cubexo,0,0) -- cycle;
\draw[gray,fill=yellow] (\XEo) -- ++(0,0,-\cubezo) -- ++(0,-\cubeyo,0) -- ++(0,0,\cubezo) -- cycle;
\draw[gray,fill=yellow] (\XEo) -- ++(-\cubexo,0,0) -- ++(0,0,-\cubezo) -- ++(\cubexo,0,0) -- cycle;

\draw[gray,fill=yellow] (\XEt) -- ++(-\cubext,0, 0) -- ++(0,-\cubeyt,0) -- ++(\cubext,0,0) -- cycle;
\draw[gray,fill=yellow] (\XEt) -- ++(0,0,-\cubezt) -- ++(0,-\cubeyt,0) -- ++(0,0,\cubezt) -- cycle;
\draw[gray,fill=yellow] (\XEt) -- ++(-\cubext,0,0) -- ++(0,0,-\cubezt) -- ++(\cubext,0,0) -- cycle;

\draw[gray,fill=yellow] (\XEtr) -- ++(-\cubextr,0, 0) -- ++(0,-\cubeytr,0) -- ++(\cubextr,0,0) -- cycle;
\draw[gray,fill=yellow] (\XEtr) -- ++(0,0,-\cubeztr) -- ++(0,-\cubeytr,0) -- ++(0,0,\cubeztr) -- cycle;
\draw[gray,fill=yellow] (\XEtr) -- ++(-\cubextr,0,0) -- ++(0,0,-\cubeztr) -- ++(\cubextr,0,0) -- cycle;


\draw[gray,fill=yellow] (\XDo) -- ++(-\cubextr,0, 0) -- ++(0,-\cubeytr,0) -- ++(\cubextr,0,0) -- cycle;
\draw[gray,fill=yellow] (\XDo) -- ++(0,0,-\cubeztr) -- ++(0,-\cubeytr,0) -- ++(0,0,\cubeztr) -- cycle;
\draw[gray,fill=yellow] (\XDo) -- ++(-\cubextr,0,0) -- ++(0,0,-\cubeztr) -- ++(\cubextr,0,0) -- cycle;

\draw[gray,fill=yellow] (\XDt) -- ++(-\cubext,0, 0) -- ++(0,-\cubeyt,0) -- ++(\cubext,0,0) -- cycle;
\draw[gray,fill=yellow] (\XDt) -- ++(0,0,-\cubezt) -- ++(0,-\cubeyt,0) -- ++(0,0,\cubezt) -- cycle;
\draw[gray,fill=yellow] (\XDt) -- ++(-\cubext,0,0) -- ++(0,0,-\cubezt) -- ++(\cubext,0,0) -- cycle;

\draw[gray,fill=yellow] (\XDtr) -- ++(-\cubexo,0, 0) -- ++(0,-\cubeyo,0) -- ++(\cubexo,0,0) -- cycle;
\draw[gray,fill=yellow] (\XDtr) -- ++(0,0,-\cubezo) -- ++(0,-\cubeyo,0) -- ++(0,0,\cubezo) -- cycle;
\draw[gray,fill=yellow] (\XDtr) -- ++(-\cubexo,0,0) -- ++(0,0,-\cubezo) -- ++(\cubexo,0,0) -- cycle;
	
	
	
	
	
	
	\node [process, left=0.5cm of NN, align=center] (warping) {warping};
	
	%\node[circle,draw=black, fill=gray, inner sep=0pt,minimum size=5pt] (b) at ($(warping) + (-2.5,0)$) {};
	
	\node[circle,draw=black, fill=gray, inner sep=0pt,minimum size=5pt, left=0.3cm of warping] (b) {};
	
	\node [process, left=0.3cm of b, align=center] (rd) {labeling \\ (vision model)};
	\node [DataInput, left=0.3cm of rd, align=center] (lidarCamera) {Lidar \&\\ camera}; 
	
	\node [process, align=center] (DRISF) at ($(rd)+(0,2.5)$) {scene flow \& \\ depth estimation};
	
	
	%\node (rv) at ($(rd)+(0,2.5)$) {range \& velocity};
	
	
	
    
    \path [arrow] (fftData.180)  -- (NN.0);
	%\path [arrow, color=green]  ($(NN.0)+(0.0,-0.5)$) -|++(0.3, -2);    
    
    
    
    \begin{pgfonlayer}{bg} 
    
     %\path[fill=yellow!20,rounded corners, draw=black!50, dashed]
           % ($(fftData.0) + (+0.4, -2.8)$) rectangle ($(NN.-90) + (-1.9, 2.3)$);
            
            %\path[fill=yellow!20,rounded corners, draw=black!50, dashed]
           % ($(fftData.0) + (+0.4, -1.2)$) rectangle ($(NN.-90) + (-1.9, 3.3)$);
            
            
            %\draw[black,fill=yellow!20, opacity=0.2, dashed] ($(-18.5,0.5)+(-4,-6)$) -- ++(47,0, 0) -- ++(0,8.5,0) -- ++(-12.5,0,0)-- ++(0,10.3,0)-- ++(-8,0,0)-- ++(0,-10.3,0) -- ++(-26.5,0,0) -- cycle;
            
            
    % draw connections
    
    \path [arrow] (NN.180)  -- (warping.0);
    \path [arrow] (warping.180)  -- (b.0);
	\path [arrow] (lidarCamera.0)  -- (rd.180); 
	\path [arrow] (rd.0)  -- (b.180);    
    
%    \path [arrow] (b.south) |-  ($(NN.-90)+(-1.5,-1.5)$) |- ($(NN.-90)+(-1.5,-0.5)$) -- ($(NN.90)+(1.5,0.7)$);
    
    %\path [draw, color=green] (b.south) |- ($(NN.180)+(0.5,-0.5)$);
%\path [arrow, color=gray] (b.south) |- ($(NN.0)+(0.5,-0.5)$) --++(0, -2);
    
%    \path [arrow, dashed] (lidarCamera.90) --++  (0,1) -| (warping.90);    
    
	%\path (fftData.west |- fftData.east)+(-0.5,0.3) node (a) {};    
 
 
 
 
 %\coordinate (warpingPoint) at ($(\x{warping}, \y{DRISF})$);
 
 
 \path [arrow, dashed] (lidarCamera.90) |- (DRISF.190);   
  \path [arrow, dashed] (DRISF.0) -| (warping.90);  
  
  
%  \path [arrow, dashed] (fftData.90) |- ($(lidarCamera.90) + (0,+3)$) --($(lidarCamera.90) + (0,+1.5)$);  
    \path [arrow, dashed] (fftData.90) |- ($(lidarCamera.90) + (0,+3)$) |-($(DRISF.170)$);   
	
                
    %\path [draw, color=green, dashed] (b.south) |- ($(NN.180)+(-0.5,-0.8)$);
    
    
    \end{pgfonlayer}
    
    
    
    %\path [draw, color=green] (b.south) |- ($(NN.180)+(0.5,-0.5)$);
    %\path [arrow, color=green]  ($(NN.0)+(0.0,-0.5)$) -|++(0.3, -2);  
    
%    \path [draw, color=green] (b.south) |- ($(NN.0)+(0.0,-0.5)$)-|++(0.3, -2);
    \path [arrow, color=green, dashed] (b.south) |- ($(NN.270)+(-0.0,-0.5)$) -- ($(NN.270)+(0.0,-0.0)$);
    
    
    \node at ($(b.-90)+(-0.4,-0.3)$) {$-$};
    \node[rotate=25] at ($(b.0)+(-1.9,-2)$) {supervision};
    
%    \node[align=right] at ($(fftData.-90)+(0.7,-0.9)$) {Radar\\ software};
    %\node[align=center] at ($(fftData)!0.5!(NN)+(0.0,+1.7)$) {Radar software};
    
    
    
%    \node at ($(NN.90)+(1,1.2)$) {backpropagation};
    
    \node[align=left] at ($(NN.90)+(1.5,-3.4)$) {error\\ backpropagation};
    
    \node[align=center] at ($(NN.90)+(0,1.1)$) {neural\\ network};
%    \node[align=center] at ($(NN.180)-(0,1.1)$) {neural\\ network};

        \node (rv) at ($(lidarCamera)+(-3.25,0)$) {$ $};
        
        
%        \node (rv) at ($(lidarCamera)!0.5!(warping)+(0,2.5)$) {range \& velocity};





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{pgfonlayer}{bg}    % select the background layer
\newcommand*{\imageHeight}{1.575cm}%
\newcommand*{\imageWidth}{1.9250cm}%
	
%\draw[dashed] ($(lidarCamera.180)+(0,-4)$)--($(fftData.0)+(0,-4)$);


\newcommand*{\frameNameE}{Class_Frame_9918}
	\newcommand*{\folder}{Results/Class/Supplement2}


    
    \node[draw=black,thick,inner sep=0pt,opacity=1] (vd_l1) at ($(lidarCamera.0)+(-1,-6)$)
        {\includegraphics[width=\imageWidth]{\folder/\frameNameE/rgb1.png}};
        
        
\node[draw=black,thick,inner sep=0pt,opacity=1] (vd_l2) at ($(rd.0)+(-2,-6)$)
    {\includegraphics[width=\imageWidth]{\folder/\frameNameE/hsv1_contrastAdjust.png}};
    
   \node[draw=black,thick,inner sep=0pt,opacity=1] (vd_l3) at ($(warping.180)+(1,-6)$)
        {\includegraphics[width=\imageWidth]{\folder/\frameNameE/hsv2_contrastAdjust.png}};
    
    
    \node[draw=black,thick,inner sep=0pt,opacity=1] (vd_l4) at ($(NN.0)+(-1,-6)$)
        {\includegraphics[width=\imageWidth]{\folder/\frameNameE/hsv4_contrastAdjust.png}};
        
        
        \node[draw=black,thick,inner sep=0pt,opacity=1] (vd_l5) at ($(fftData.0)+(-0.5,-6)$)
        {\includegraphics[width=\imageWidth]{\folder/\frameNameE/RDMap3.png}};
        
    
    %%%%%%
   % \draw[dashed] ($(lidarCamera.0)+(0.2,0)$)--($(vd_l1.39.3)+(0,0)$);
    %\draw[dashed] ($(lidarCamera.0)+(0.2,0)$)--($(vd_l1.140.7)+(0,0)$);
    
    
  
  \fill[gray, ultra thick, opacity=0.15] ($(lidarCamera.0)+(0.2,0)$) -- ($(vd_l1.39.3)+(0,0)$) -- ($(vd_l1.140.7)+(0,0)$) -- cycle;
    
    
    
    %\draw[dashed] ($(rd.0)+(0.2,0)$)--($(vd_l2.39.3)+(0,0)$);
    %\draw[dashed] ($(rd.0)+(0.2,0)$)--($(vd_l2.140.7)+(0,0)$);
    \fill[gray, ultra thick, opacity=0.15] ($(rd.0)+(0.2,0)$) -- ($(vd_l2.39.3)+(0,0)$) -- ($(vd_l2.140.7)+(0,0)$) -- cycle;
    
    
    
    %\draw[dashed] ($(warping.180)+(-0.2,0)$)--($(vd_l3.39.3)+(0,0)$);
    %\draw[dashed] ($(warping.180)+(-0.2,0)$)--($(vd_l3.140.7)+(0,0)$);
    \fill[gray, ultra thick, opacity=0.15] ($(warping.180)+(-0.2,0)$) -- ($(vd_l3.39.3)+(0,0)$) -- ($(vd_l3.140.7)+(0,0)$) -- cycle;
    
    
    
    %\draw[dashed] ($(warping.0)+(0.2,0)$)--($(vd_l4.39.3)+(0,0)$);
    %\draw[dashed] ($(warping.0)+(0.2,0)$)--($(vd_l4.140.7)+(0,0)$);
    \fill[gray, ultra thick, opacity=0.1] ($(warping.0)+(0.4,0)$) -- ($(vd_l4.39.3)+(0,0)$) -- ($(vd_l4.140.7)+(0,0)$) -- cycle;
    
    
    
    %\draw[dashed] ($(fftData.180)+(-0.2,0)$)--($(vd_l5.39.3)+(0,0)$);
    %\draw[dashed] ($(fftData.180)+(-0.2,0)$)--($(vd_l5.140.7)+(0,0)$);
    \fill[gray, ultra thick, opacity=0.15] ($(fftData.180)+(-0.4,0)$) -- ($(vd_l5.39.3)+(0,0)$) -- ($(vd_l5.140.7)+(0,0)$) -- cycle;
    
    \end{pgfonlayer}
   
    
\end{tikzpicture}


==> Flowchart_nn_and_gt3_.tex <==
% Flowchart of Lidar2RAdar generation
\tikzstyle{decision} = [diamond, draw, fill=gray!20, 
    text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=gray!20, 
    text width=15em, text centered, minimum height=4em]
    \tikzstyle{blockstart} = [rectangle, draw, fill=blue!20, 
    text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{line2} = [draw]
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
    \tikzstyle{block2} = [rectangle, draw, fill=gray!20, 
    text width=13em, text centered, minimum height=4em]
  %\centering 
  
  
  
\tikzstyle{DataInput} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=1cm, text centered, draw=black, fill=gray!30]  

\tikzstyle{process} = [rectangle, minimum width=1.0cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
   
\tikzstyle{arrow} = [draw, -latex',thick]
\tikzstyle{arrowDashed} = [draw, -latex',thick, dashed]


\tikzstyle{diff} = [circle, minimum width=1.0cm, minimum height=1cm, text centered, draw=black, fill=gray!30]


\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)


\begin{tikzpicture}[node distance = 2cm, auto, scale=0.5]

	\node [DataInput, align=center] (fftData) {radar}; 
	
	
    
    \pgfmathsetmacro{\xshift}{-4.3}
    
    \pgfmathsetmacro{\cubexo}{0.2}
    \pgfmathsetmacro{\cubeyo}{1.5}
	\pgfmathsetmacro{\cubezo}{1.5}
	
	\pgfmathsetmacro{\cubext}{0.2}
    \pgfmathsetmacro{\cubeyt}{1.25}
	\pgfmathsetmacro{\cubezt}{1.25}
	
	\pgfmathsetmacro{\cubextr}{0.2}
    \pgfmathsetmacro{\cubeytr}{1.0}
	\pgfmathsetmacro{\cubeztr}{1.0}
	
	\newcommand\XEo{-5.5,0.5,0}
	\newcommand\XEt{-5,0.375,0}
	\newcommand\XEtr{-4.5, 0.25, 0}
	
	\newcommand\XDo{-4, 0.25, 0}
	\newcommand\XDt{-3.5,0.375,0}
	\newcommand\XDtr{-3,0.5,0}

\draw[gray,fill=yellow] ($(\XEo) + (\xshift,0)$) -- ++(-\cubexo,0, 0) -- ++(0,-\cubeyo,0) -- ++(\cubexo,0,0) -- cycle;
\draw[gray,fill=yellow] ($(\XEo) + (\xshift,0)$) -- ++(0,0,-\cubezo) -- ++(0,-\cubeyo,0) -- ++(0,0,\cubezo) -- cycle;
\draw[gray,fill=yellow] ($(\XEo) + (\xshift,0)$) -- ++(-\cubexo,0,0) -- ++(0,0,-\cubezo) -- ++(\cubexo,0,0) -- cycle;

\draw[gray,fill=yellow] ($(\XEt) + (\xshift,0)$) -- ++(-\cubext,0, 0) -- ++(0,-\cubeyt,0) -- ++(\cubext,0,0) -- cycle;
\draw[gray,fill=yellow] ($(\XEt) + (\xshift,0)$) -- ++(0,0,-\cubezt) -- ++(0,-\cubeyt,0) -- ++(0,0,\cubezt) -- cycle;
\draw[gray,fill=yellow] ($(\XEt) + (\xshift,0)$) -- ++(-\cubext,0,0) -- ++(0,0,-\cubezt) -- ++(\cubext,0,0) -- cycle;

\draw[gray,fill=yellow] ($(\XEtr) + (\xshift,0)$) -- ++(-\cubextr,0, 0) -- ++(0,-\cubeytr,0) -- ++(\cubextr,0,0) -- cycle;
\draw[gray,fill=yellow] ($(\XEtr) + (\xshift,0)$) -- ++(0,0,-\cubeztr) -- ++(0,-\cubeytr,0) -- ++(0,0,\cubeztr) -- cycle;
\draw[gray,fill=yellow] ($(\XEtr) + (\xshift,0)$) -- ++(-\cubextr,0,0) -- ++(0,0,-\cubeztr) -- ++(\cubextr,0,0) -- cycle;


\draw[gray,fill=yellow] ($(\XDo) + (\xshift,0)$) -- ++(-\cubextr,0, 0) -- ++(0,-\cubeytr,0) -- ++(\cubextr,0,0) -- cycle;
\draw[gray,fill=yellow] ($(\XDo) + (\xshift,0)$) -- ++(0,0,-\cubeztr) -- ++(0,-\cubeytr,0) -- ++(0,0,\cubeztr) -- cycle;
\draw[gray,fill=yellow] ($(\XDo) + (\xshift,0)$) -- ++(-\cubextr,0,0) -- ++(0,0,-\cubeztr) -- ++(\cubextr,0,0) -- cycle;

\draw[gray,fill=yellow] ($(\XDt) + (\xshift,0)$) -- ++(-\cubext,0, 0) -- ++(0,-\cubeyt,0) -- ++(\cubext,0,0) -- cycle;
\draw[gray,fill=yellow] ($(\XDt) + (\xshift,0)$) -- ++(0,0,-\cubezt) -- ++(0,-\cubeyt,0) -- ++(0,0,\cubezt) -- cycle;
\draw[gray,fill=yellow] ($(\XDt) + (\xshift,0)$) -- ++(-\cubext,0,0) -- ++(0,0,-\cubezt) -- ++(\cubext,0,0) -- cycle;

\draw[gray,fill=yellow] ($(\XDtr) + (\xshift,0)$) -- ++(-\cubexo,0, 0) -- ++(0,-\cubeyo,0) -- ++(\cubexo,0,0) -- cycle;
\draw[gray,fill=yellow] ($(\XDtr) + (\xshift,0)$) -- ++(0,0,-\cubezo) -- ++(0,-\cubeyo,0) -- ++(0,0,\cubezo) -- cycle;
\draw[gray,fill=yellow] ($(\XDtr) + (\xshift,0)$) -- ++(-\cubexo,0,0) -- ++(0,0,-\cubezo) -- ++(\cubexo,0,0) -- cycle;
	
	
	
	
	
	
	\node [process, left=0.5cm of fftData, align=center] (warping) {warping};
	
	%\node[circle,draw=black, fill=gray, inner sep=0pt,minimum size=5pt] (b) at ($(warping) + (-2.5,0)$) {};
	
	\node[circle,draw=black, fill=gray, inner sep=0pt,minimum size=5pt, left=0.3cm of warping] (b) {};
	
	\node [process, left=0.3cm of b, , align=center, opacity=.0] (NN) {Neural\\ Network};
	
	\node [process, left=0.3cm of NN, align=center] (rd) {feature generation \\ (vision model)};
	\node [DataInput, left=0.3cm of rd, align=center] (lidarCamera) {Lidar \&\\ camera}; 
	
	\node [process, align=center] (DRISF) at ($(rd)+(0,2.8)$) {scene flow \& \\ depth estimation};
	
	
	%\node (rv) at ($(rd)+(0,2.5)$) {range \& velocity};
	
	
	
    
    \path [arrow] (fftData.180)  -- (warping.0);
	%\path [arrow, color=gray, green]  ($(NN.180)+(-0.4,-0.5)$) -|++(0.0, -2);    
	
	%\path [arrow, color=gray, green]  ($(NN.180)+(-0.4,-0.5)$) -|++(0.0, -2); 
	\path [arrow, color=green, dashed] (b.south) |- ($(NN.270)+(0,-0.5)$) -- ($(NN.270)+(0,-0.0)$);  
%	 \path [arrow, color=green, dashed] (b.south) |- ($(NN.270)+(-0.0,-0.5)$) -- ($(NN.270)+(0.0,-0.0)$); 
    
    
    
    \begin{pgfonlayer}{bg} 
    
     %\path[fill=yellow!20,rounded corners, draw=black!50, dashed]
           % ($(fftData.0) + (+0.4, -2.8)$) rectangle ($(NN.-90) + (-1.9, 2.3)$);
            
            %\path[fill=yellow!20,rounded corners, draw=black!50, dashed]
           % ($(fftData.0) + (+0.4, -1.2)$) rectangle ($(NN.-90) + (-1.9, 3.3)$);
            
            
            %\draw[black,fill=yellow!20, opacity=0.2, dashed] ($(-18.5,0.5)+(-4,-6)$) -- ++(47,0, 0) -- ++(0,8.5,0) -- ++(-12.5,0,0)-- ++(0,10.3,0)-- ++(-8,0,0)-- ++(0,-10.3,0) -- ++(-26.5,0,0) -- cycle;
            
            
    % draw connections
    
    \path [arrow] (NN.180)  -- (b.180);
    \path [arrow] (warping.180)  -- (b.0);
	\path [arrow] (lidarCamera.0)  -- (rd.180); 
	\path [arrow] (rd.0)  -- (NN.180);    
    
%    \path [arrow] (b.south) |-  ($(NN.-90)+(-1.5,-1.5)$) |- ($(NN.-90)+(-1.5,-0.5)$) -- ($(NN.90)+(1.5,0.7)$);
    
    %\path [draw, color=green] (b.south) |- ($(NN.180)+(-0.4,-0.5)$);
%\path [arrow, color=gray] (b.south) |- ($(NN.0)+(0.5,-0.5)$) --++(0, -2);
    
%    \path [arrow, dashed] (lidarCamera.90) --++  (0,1) -| (warping.90);    
    
	%\path (fftData.west |- fftData.east)+(-0.5,0.3) node (a) {};    
 
 
 
 
 %\coordinate (warpingPoint) at ($(\x{warping}, \y{DRISF})$);
 
 
 \path [arrow, dashed] (lidarCamera.90) |- (DRISF.190);   
  \path [arrow, dashed] (DRISF.0) -| (warping.90);  
  
  
%  \path [arrow, dashed] (fftData.90) |- ($(lidarCamera.90) + (0,+3.2)$) --($(lidarCamera.90) + (0,+1.5)$);   
\path [arrow, dashed] (fftData.90) |- ($(lidarCamera.90) + (0,+3.2)$) |-($(DRISF.170)$);
	
                
    
   
    
   
            
            
    \end{pgfonlayer}
    
    \node at ($(b.-90)+(-0.3,+0.5)$) {$-$};
    \node[rotate=-25] at ($(b.0)+(+1.7,-2)$) {supervision};
    
%    \node[align=right] at ($(fftData.-90)+(0.7,-0.9)$) {Radar\\ software};
    %\node[align=center] at ($(fftData)!0.5!(NN)+(0.0,+1.7)$) {Radar software};
    
    
    
%    \node at ($(NN.90)+(1,1.2)$) {backpropagation};
    
    \node[align=right] at ($(NN.90)+(-2.6,-3.2)$) {error\\ backpropagation};
    
    \node[align=center] at ($(NN.90)+(0,1.05)$) {neural\\ network};
%    \node[align=center] at ($(NN.180)-(0,1.1)$) {neural\\ network};

        \node (rv) at ($(lidarCamera)+(-3.25,0)$) {$ $};
        
        
%        \node (rv) at ($(lidarCamera)!0.5!(warping)+(0,2.5)$) {range \& velocity};
        
    
   
    
\end{tikzpicture}

